Joint Upper & Lower Bound Normalization for IR Evaluation

In this paper, we present a novel perspective towards IR evaluation by proposing a new family of evaluation metrics where the existing popular metrics (e.g., nDCG, MAP) are customized by introducing a query-specific lower-bound (LB) normalization term. While original nDCG, MAP etc. metrics are normalized in terms of their upper bounds based on an ideal ranked list, a corresponding LB normalization for them has not yet been studied. Specifically, we introduce two different variants of the proposed LB normalization, where the lower bound is estimated from a randomized ranking of the corresponding documents present in the evaluation set. We next conducted two case-studies by instantiating the new framework for two popular IR evaluation metric (with two variants, e.g., DCG_UL_V1,2 and MSP_UL_V1,2 ) and then comparing against the traditional metric without the proposed LB normalization. Experiments on two different data-sets with eight Learning-to-Rank (LETOR) methods demonstrate the following properties of the new LB normalized metric: 1) Statistically significant differences (between two methods) in terms of original metric no longer remain statistically significant in terms of Upper Lower (UL) Bound normalized version and vice-versa, especially for uninformative query-sets. 2) When compared against the original metric, our proposed UL normalized metrics demonstrate higher Discriminatory Power and better Consistency across different data-sets. These findings suggest that the IR community should consider UL normalization seriously when computing nDCG and MAP and more in-depth study of UL normalization for general IR evaluation is warranted.

==> sections/6ERR.tex <==

% \setlength{\parskip}{0.5em}
\subsection{Case Study 3: ERR with Joint Upper \& Lower Bound Normalization}
This section demonstrates our last case study metric: $ERR$. We first introduced the random ranking $ERR$ computation and then present our implications.





% \begin{table}[!htb]
% 	\begin{center}
	   
% 		\begin{tabular}{c||c|c|c|c}\hline
% 		& \multicolumn{4}{c} {\textbf{Kendall's $\uptau$}}\\\cline{2-5}
% 		{\bf Data-set} & {\bf version }& \textbf{All} &{\bf Closest} & {\bf Furthest} \\\hline\hline
		
% 		\multirow{4}{*}{\bf MSLR-WEB30K} & ERR and V1 & 1 & 0.7857 &    1 \\\cline{2-5}
		
% 		 & ERR and V2 & 0.9285 &0.5 & 1 \\\cline{2-5}
		
% 		& nERR and V1 & 1 & 1 &    1 \\\cline{2-5}
		
% 		& nERR and V2 & 0.9285 &0.714 & 1 \\\hline\hline
		
	
		
% 		\multirow{4}{*}{\bf MQ2007} & ERR and V1 & 0.9285 & 0.785 &    1 \\\cline{2-5}
		
% 		 & ERR and V2 & 0.8571 &0.214 & 0.571 \\\cline{2-5}
		
% 		& nERR and V1 & 0.9285 & 1 &    1 \\\cline{2-5}
		
% 		& nERR and V2 &1  & 0 & 0.571 \\\hline
% 		\end{tabular}

% 		\caption{Kendall's $\uptau$ rank correlations between LETOR method ranks based on $ERR$, $nERR$ and two $ERR^{UL}$ in \textit{All} \textit{Uninformative 1000} or \textit{Ideal 1000} query sets. \Dongji{DONE}}
% 		\label{table:kendall_conflict_ERR_1000}
% 		\end{center}
% 		\vspace{-3mm}
% \end{table}







% \begin{table}[!htb]
% 	\begin{center}
	   
% 		\begin{tabular}{c||c|c|c|c}\hline
% 		& \multicolumn{4}{c} {\textbf{Conflict Cases}}\\\cline{2-5}
% 		{\bf Data-set} & {\bf version }& \textbf{All} & {\bf uniform} & {\bf Ideal} \\\hline\hline
		
% 		\multirow{4}{*}{\bf MSLR-WEB30K} & ERR and V1 & 16 & 15  & 0    \\\cline{2-5}
		
% 		& ERR and V2 & 16 & 53 & 1 \\\cline{2-5}
		
% 		& nERR and V1 & 4 & 9 & 0  \\\cline{2-5}
% 		& nERR and V2 & 4 & 53 & 1 \\\hline\hline
		
	
		
% 		\multirow{4}{*} {\bf MQ2007} & ERR and V1 & 1&  0 & 4  \\\cline{2-5}
		
% 		 & ERR and V2 & 8 &  11 &  14 \\\cline{2-5}
% 		 & nERR and V1 & 0 & 0 &  1 \\\cline{2-5}
% 		 & nERR and V2 & 7 & 11 &  13\\\hline\hline
	
% 		\end{tabular}

% 		\caption{We used Student's t-test to verify whether statistically significant difference occurred between a pair of LETOR methods while using $ERR$ and $ERR^{U L}$ and counted the total number of disagreements on ``MSLR-WEB30K'' and ``MQ2007'' data-set \Dongji{DONE}}
% 		\label{table:statistical_test_conflict_all_query_ERR}
% 		\end{center}
% 		\vspace{-3mm}
% \end{table}






% \begin{table}[!htb]
% 	\begin{center}
	   
% 		\begin{tabular}{c||c|c|c|c}\hline
% 		& \multicolumn{4}{c} {\textbf{Number of Stat-Sig difference}}\\\cline{2-5}
% 		{\bf Data-set} & {\bf version }& {\bf All} &{\bf uninform} & {\bf Ideal} \\\hline\hline
		
% 		\multirow{4}{*}{\bf MSLR-WEB30K} & ERR & 140  & 118 &  140   \\\cline{2-5}
		
% 		& nERR & 137 & 116 & 135 \\\cline{2-5}
% 		& V1 &  140 & 119 & 139\\\cline{2-5}
% 		& V2 & 140 & 86 & 140 \\\hline\hline
		
	
		
% 		\multirow{4}{*} {\bf MQ2007} & ERR & 36 & 35  &  36 \\\cline{2-5}
		
% 		& nERR & 35 &  35& 41 \\\cline{2-5}
% 		& V1 &  35 &  35& 40  \\\cline{2-5}
		
% 		& V2 & 42 & 38 & 50 \\\hline
	
% 		\end{tabular}
		
		
% 		\caption{Total number of statistically significant differences detected based on $ERR$ and $ERR^{UL}$ on all queries, 1000 \textit{uninformative} queries and \textit{Ideal} queries from the ``MSLR-WEB30K'' and `` MQ2007 '' data-set. \Dongji{DONE}}
%         \label{table:student_discriminative_MSLR_WEB30K_ERR}
% 		\end{center}
% 		\vspace{-3mm}
% \end{table}




% \begin{table}[!htb]
% 	\begin{center}
	   
% 		\begin{tabular}{c||c|c|c}\hline
% 		& \multicolumn{3}{c} {\textbf{Swap Rate}  }\\\cline{2-4}
% 		{\bf Metric}  & {\bf All} &  {\bf uninform} & {\bf Ideal}\\\hline\hline
		
% 		{\bf ERR} & 0.39 & 0.2857   &  0.464 \\\hline
		
% 		{\bf nERR} & 0.35 & 0.357  &  0.464 \\\hline
		
% 		$\bf ERR^{UL}_{V_1}$ &0.39  & 0.357  & 0.464 \\\hline
% 		$\bf ERR^{UL}_{V_2}$ & 0.32 &  0.392 & 0.464\\\hline
	
% 		\end{tabular}
		
		
% 		\caption{Swap rates between method ranks on \textit{uninform }/\textit{Ideal} queries across ``MSLR-WEB30K'' and ``MQ2007''  data-sets.\Dongji{DONE}}
%         \label{table:Swap_Rate_Consistency_closest_furthest_ERR}
% 		\end{center}
% 		\vspace{-3mm}
% \end{table}


% \begin{table}[!htb]
% 	\begin{center}
	   
% 		\begin{tabular}{c||c|c}\hline
% 		& \multicolumn{2}{c} {\textbf{Swap Rate}  }\\\cline{2-3}
% 		{\bf Metric}  & {\bf MSLR-WEB30K} & {\bf MQ2007}\\\hline\hline
% 		{\bf ERR} &   0.14& 0.25  \\\hline
% 		{\bf nERR} &   0.25& 0.39  \\\hline
% 		$\bf ERR^{UL}_{V_1}$ &   0.25 & 0.39
% 		\\\hline
		
% 		$\bf ERR^{UL}_{V_2}$ & 0.39    &  0.32\\\hline
	
% 		\end{tabular}
% 		\caption{Swap rates between method ranks on \textit{MSLR-WEB30K}/\textit{MQ2007} data-sets across ``uninform'' and ``Ideal'' query collections. \Dongji{DONE}}
%         \label{table:Swap_Rate_Consistency_across_dataset_ERR}
% 		\end{center}
% 		\vspace{-3mm}
% \end{table}


\subsubsection{\textbf{Lower-Bound of ERR (ERR of Random Ranking):}} We again leverage the idea of random ranking to compute a more realistic lower-bound for $ERR$, i.e., the expected $ERR$ in case of random ranking. Thus, $RLB[ERR@k]$ is essentially the expected $ERR@k$ computed based on a randomly ranked list and we will use the terms $E[ERR@k]$ and $RLB[ERR@k]$ interchangeably throughout the paper. Mathematically, $E[ERR@k]$ can be expressed as follows:


\vspace{-3mm}

\begin{align*}
E[ERR@k] &= E\left[\sum_{r=1}^{k} \frac{1}{r} \prod_{i=1}^{r-1}(1-R_{i})\cdot R_{r}\right] 
= \sum_{r=1}^{k}\frac{1}{r} \cdot E\left[\prod_{i=1}^{r-1} (1- R_{i}) \cdot R_{r}\right]
\end{align*}
\vspace{-3mm}

Here, $k$ is the cut-off depth, $r$ is the current position, $i$ represents all positions above rank $r$. The computation of $E[ERR@k]$ actually relies on the computation of $E\left[\prod_{i=1}^{r-1} (1- R_{i}) \cdot R_{r}\right]$, where, $R_{i}$ and $R_{r}$ are the expected relevance labels of the previous documents at position $i$ (ranging from $0$ to $r-1$) and current document at position $r$, respectively. Assuming that relevance labels of previous documents are independent of the relevance label of the current document, we can break the above expectation into a product of two independent expectations.

\vspace{-2mm}
\begin{equation*}
    E[ERR@k] = \sum_{r=1}^{k}\frac{1}{r} \cdot \left(\prod_{i=1}^{r-1} E\left[(1- R_{i})\right]\right)\cdot E[R_{r}]
\end{equation*}
\vspace{-3mm}

Now, we need to compute two expectations: $E[R_{r}]$ and $E[(1- R_{i})]$. Since $R_{i}$ and $R_{r}$ are essentially the same expectation for two different positions, without loss of generality, we will only show how to estimate $E[R_{r}]$. %

\vspace{-2mm}
\begin{align*}
\boldsymbol{E[R_{r}]} &= \sum_{j=1}^{i} (j)\cdot Pr(R_{r} = j)
= \sum_{j=1}^{i} (j) \cdot \left[\frac{^{n_j}_{}{P_1} \cdot ^{n-1}P_{k-1}  }{^{n}{P_k}}\right] \\
&= (j) \sum_{j=1}^{i}  \left[\frac{ \frac{n_j !} {(n_j - 1)!} \cdot \frac{(n-1)!}{(n-k)!} }    {\frac{n!}{(n-k)!}}\right] 
= \sum_{j=1}^{i} (j) \cdot  \left(\frac{n_j}{n}\right)  
= \sum_{j=1}^{i} (j) \cdot Pr(R=j) = \boldsymbol{E[R]} \\
\vspace{-5mm}
\end{align*}

Here, $^{n}_{}{P_r}$ denotes the total number of permutations one can consider by arranging $r$ documents from a collection of $n$ documents. Definitions of $Pr(j)$, $n$ and $n_j$ are identical to section \ref{sec:Expected4nDCG} and hence, we omit their explanations here. In the same way, proof of $E[(1- R_{i})]=E[1 - R]$ is trivial. Thus, the final formula to compute the expectation of $ERR@k$ can be expressed by the following equation.

\begin{equation*}
    E[ERR@k] = \sum_{r=1}^{k}\frac{1}{r} \cdot \left(\prod_{i=1}^{r-1} E\left[(1- R)\right]\right) \cdot E[R]
\end{equation*}


\begin{table}
	
    \begin{center}
    \begin{tabular}{c|c|c|c|c|c||c|c|c|c|c}\hline
         &  \multicolumn{5}{c||}{$ERR@$} & \multicolumn {5}{c}{$nERR@$}\\\cline{2-11}
         {\bf Method} & {\bf 5} & {\bf 10} & {\bf 15} & {\bf 20} & {\bf 30} & {\bf 5} & {\bf 10} & {\bf 15} & {\bf 20} & {\bf 30}\\\hline\hline
         
         ARank & 0.1761  & 0.1948  & 0.2022 & 0.2059 & \textbf{0.2094} & 0.2502  & 0.2782  & 0.2911 & 0.2983 & 0.3057\\\hline
         
         LNet & 0.1012  & 0.1224 & 0.1319  & 0.1368  & \textbf{0.1414} & 0.183  & 0.2138 & 0.2288  & 0.2375  & 0.2458 \\\hline
         
         RBoost & 0.203   & 0.2258  & 0.2336  & 0.2371  & \textbf{0.2399} & 0.3566   & 0.3858  & 0.3979  & 0.404  & 0.4095 \\\hline
         
         RF & 0.2801  & 0.3017  & 0.308  & 0.3106  & \textbf{0.3127} & 0.4552  & 0.4827  & 0.4927  & 0.4975  & 0.5018 \\\hline
         
         RNet & 0.1067  & 0.1278  & 0.1371  & 0.142  & \textbf{0.1464} & 0.1899  & 0.2203  & 0.2353  & 0.2438  & 0.252\\\hline
         
         CA & 0.3082  & 0.3272  & 0.3332  & 0.3358  & \textbf{0.3381} & 0.4875  & 0.5107  & 0.5203  & 0.5251  & 0.5297 \\\hline
         
         L2LR & 0.1428 & 0.1669 & 0.176 & 0.1804 & \textbf{0.1841} & 0.2348 & 0.2694 & 0.2851 & 0.2934 & 0.3009 \\\hline
         
         LMART &  0.3342  &  0.3524 &  0.3581  &  0.3605 & \textbf{0.3625} &  0.5114  &  0.5346 &  0.544  &  0.5486 & 0.553 \\\hline
    \end{tabular}
    
    \caption{Relative ERR and nERR performances of different LETOR methods for variable $k$ MSLR-WEB30K \Dongji{DONE} }
    
    \label{table:ERRandnERR_averageVaryKMSLR_WEB30K}
    \end{center}
 
    \vspace{-2mm}
\end{table}



\begin{table}
    \begin{center}
    \begin{tabular}{c|c|c|c|c|c||c|c|c|c|c}\hline
         &  \multicolumn{5}{c||}{$ERR@$} & \multicolumn {5}{c}{$nERR@$}\\\cline{2-11}
         {\bf Method} & {\bf 5} & {\bf 10} & {\bf 15} & {\bf 20} & {\bf 30} & {\bf 5} & {\bf 10} & {\bf 15} & {\bf 20} & {\bf 30}\\\hline\hline
         ARank & 0.056  & 0.067  & 0.073 & 0.075 & 0.079 & \textbf{0.267 } & 0.289  & 0.304 & 0.314 & 0.328\\\hline
         LNet & 0.082  & 0.084 & 0.099  & 0.102  & 0.105 & \textbf{0.388}  & 0.41 & 0.423  & 0.432  & 0.443 \\\hline
         RBoost & 0.084   & 0.096  & 0.102  & 0.104  & 0.107 & \textbf{0.392}   & 0.414  & 0.428  & 0.437  & 0.447 \\\hline
         RF & 0.089  & 0.101  & 0.106  & 0.108  & 0.111 & \textbf{0.413}  & 0.432  & 0.444  & 0.453  & 0.463 \\\hline
         RNet & 0.081  & 0.093  & 0.099  & 0.101  & 0.104 & \textbf{0.383}  & 0.407  & 0.421  & 0.43  & 0.441\\\hline
         CA & 0.084  & 0.097  & 0.102  & 0.104  & 0.107 & \textbf{0.397}  & 0.418  & 0.431  & 0.439  & 0.449 \\\hline
         L2LR & 0.084 & 0.096 & 0.101 & 0.104 & 0.107 & \textbf{0.396} & 0.416 & 0.429 & 0.438 & 0.449 \\\hline
         LMART &  0.081  &  0.094 &  0.099  &  0.102 & 0.104 & \textbf{ 0.387}  &  0.411 &  0.424  &  0.433 & 0.443 \\\hline
    \end{tabular}
    \caption{Relative ERR and nERR performances of different LETOR methods for variable $k$ MQ2007  \Dongji{DONE}}
    \label{table:ERRandnERR_averageVaryKMQ2007}
    \end{center}
    \vspace{-2mm}
\end{table}


\vspace{-4mm}



\begin{table*}
	\begin{adjustbox}{width=\linewidth}
		\begin{tabular}{c|c|c|c|c|c||c|c|c|c|c}\hline
		& \multicolumn{5}{c||} {$ERR^{U L}_{V_1}@$} & \multicolumn {5}{c||} {$ERR^{U L}_{V_2}@$}  \\\cline{2-11}
		{\bf Method} & {\bf 5} & {\bf 10} & {\bf 15} & {\bf 20} & {\bf 30} & {\bf 5} & {\bf 10} & {\bf 15} & {\bf 20} & {\bf 30} \\\hline\hline
		ARank & 0.1823  & 0.1933  & 0.1979 & 0.2003 & \textbf{0.2027} & -0.1467 & -0.0587  & -0.0231  & -0.0034 & 0.0166\\\hline
		
		LNet & 0.1159  & 0.1303  & 0.1374  & 0.1414  & \textbf{0.1451} & -0.1809  & -0.0936  & -0.0579  & -0.0383 & -0.0226  \\\hline
		
		RBoost & 0.2674   & 0.2806 & 0.2851 & 0.2868  & \textbf{0.2878} & 0.1733  & 0.2205 & 0.2359  & 0.2431  & 0.2486 \\\hline
		
		RF & 0.3589  & 0.3699  & 0.3722  & 0.3725  & \textbf{0.3722} & 0.3137  & 0.3556  & 0.3664  & 0.3711  & 0.3744 \\\hline
		
		RNet & 0.1215  & 0.1357  & 0.1426 & 0.1465  & \textbf{0.1501} & -0.1653 & -0.0796 & -0.044 & -0.0249 & -0.0095 \\\hline
		
		CA & 0.3898 & 0.3967 & 0.3984  & 0.3987  & \textbf{0.3985} & 0.3473 & 0.384  & 0.3961  & 0.4018  & 0.4067 \\\hline
		
		L2LR & 0.1616 & 0.1785  & 0.1858  & 0.1894  & \textbf{0.1922} & -0.0976  & 0.0008  & 0.0402  & 0.0609  & 0.0777  \\\hline
		
		LMART &  0.4131  &  0.4198  &  0.4212 &  0.4213  &  \textbf{0.4209 }&  0.3732 & 0.4126 &  0.4241 &  0.4296  &  0.4343 \\\hline
		
		\end{tabular}
		\end{adjustbox}
		\caption{Upper \& Lower Bound Normalization ERR results for different LETOR methods for variable $k$ on \textbf{``MSLR-WEB30K''} \Dongji{DONE}}
		\label{table:UL-ERR_V1_averageVaryK_MSLR}
		
    % \vspace{-2mm}
    
    
    	\begin{adjustbox}{width=\linewidth}
		\begin{tabular}{c|c|c|c|c|c||c|c|c|c|c}\hline
		& \multicolumn{5}{c||} {$ERR^{U L}_{V_1}@$} & \multicolumn {5}{c||} {$ERR^{U L}_{V_2}@$}  \\\cline{2-11}
		{\bf Method} & {\bf 5} & {\bf 10} & {\bf 15} & {\bf 20} & {\bf 30} & {\bf 5} & {\bf 10} & {\bf 15} & {\bf 20} & {\bf 30} \\\hline\hline
		ARank & 0.1823  & 0.1905  & 0.196 & 0.1998 & 0.2053 & \textbf{-0.1405} & -0.0584  & -0.0139  & 0.0135 & 0.0525\\\hline
		LNet & 0.2868  & 0.2942  & 0.2991  & 0.3023  & 0.3052 & \textbf{0.1181}  & 0.192  & 0.2236  & 0.246 & 0.266  \\\hline
		RBoost & 0.2889   & 0.297 & 0.3027 & 0.3057  & 0.3079 &\textbf{ 0.1396}  & 0.1984 & 0.2363  & 0.2576  & 0.2757 \\\hline
		RF & 0.3061  & 0.3118  & 0.3163  & 0.3189  & 0.3212 & \textbf{0.1776 } & 0.2332  & 0.2647  & 0.2868  & 0.308 \\\hline
		RNet & 0.2836  & 0.2924  & 0.2978 & 0.3008  & 0.3038 & \textbf{0.1105 }& 0.1832 & 0.22 & 0.2413 & 0.2609 \\\hline
		CA & 0.2933 & 0.3004 & 0.3054  & 0.308  & 0.3106 &\textbf{ 0.1411} & 0.2097  & 0.2458  & 0.2593  & 0.2789 \\\hline
		L2LR & 0.2919 & 0.2992  & 0.3038  & 0.3065  & 0.3094 & \textbf{0.1368}  & 0.2023  & 0.2385  & 0.2584  & 0.2813  \\\hline
		LMART &  0.2829  &  0.2935  &  0.298 &  0.3012  &  0.3037 &  \textbf{0.1321 }& 0.2052 &  0.2311 &  0.2541  &  0.272 \\\hline
		\end{tabular}
		\end{adjustbox}
		\caption{Upper \& Lower Bound Normalization ERR results for different LETOR methods for variable $k$ on \textbf{``MQ2007''}  \Dongji{DONE}}
		\label{table:UL-ERR_V1_averageVaryK_MQ2007}
		
\end{table*}	




\subsubsection{\bf UL-normalized \textit{ERR} yields different rankings compare to Original \textit{ERR} for \textit{Uninformative} query-set:} 
Table~\ref{table:kendall_conflict_ERR} shows the Kendall's $\uptau$ rank correlations between two rankings  induced by $ERR$, $nERR$ and $ERR^{UL}$ scores in \textit{All}, \textit{Uninformative} or \textit{Ideal} query collections for the two data-sets. 
Noted that $nERR$ is only upper bound normalized $ERR$ which the upper bound is calculated based on an ideal ranking result.
We first look at ``MSLR-WEB30K'' data-set. While using all query set, $ERR^{U L}_{V_2}$ generate different ranking compared with $ERR$ and $nERR$ (Kendall's  $\uptau$ are $0.9285$). Then we focuse on \textit{uninformative} query set, both two UL-bound normalized $ERR$ versions are not identical to original $ERR$. However, if we compare them with $nERR$, only $ERR^{U L}_{V_2}$ generate different ranking (Kendall's  $\uptau$ is $0.714$). Finally, for all pair comparison in $ideal$ query set, there is no difference in terms of Kendall's  $\uptau$ results. 
Next we move to the results at ``MQ2007''. Still we can find that the difference between each pair is more significant while using \textit{uninformative}(lower Kendall's  $\uptau$) compared with the same in \textit{Ideal} query set, suggesting our UL bound normalization has more impact for \textit{uninformative} query set. One interesting point is while we compare the $nERR$ with $ERR^{U L}_{V_2}$, their correlation in \textit{uninformative} is \textbf{0}.

\begin{table}[!htb]
	\begin{center}
	   
		\begin{tabular}{c||c|c|c|c}\hline
		& \multicolumn{4}{c} {\textbf{Kendall's $\uptau$}}\\\cline{2-5}
		{\bf Data-set} & {\bf version }& \textbf{All} &{\bf uninform} & {\bf Ideal} \\\hline\hline
		
		\multirow{4}{*}{\bf MSLR-WEB30K} & ERR and V1 & 1 & 0.7857 &    1 \\\cline{2-5}
		
		 & ERR and V2 & 0.9285 &0.5 & 1 \\\cline{2-5}
		
		& nERR and V1 & 1 & 1 &    1 \\\cline{2-5}
		
		& nERR and V2 & 0.9285 &0.714 & 1 \\\hline\hline
		
	
		
		\multirow{4}{*}{\bf MQ2007} & ERR and V1 & 0.9285 & 0.785 &    1 \\\cline{2-5}
		
		 & ERR and V2 & 0.8571 &0.214 & 0.571 \\\cline{2-5}
		
		& nERR and V1 & 0.9285 & 1 &    1 \\\cline{2-5}
		
		& nERR and V2 &1  & 0 & 0.571 \\\hline
		\end{tabular}

		\caption{Kendall's $\uptau$ rank correlations between LETOR method ranks based on $ERR$, $nERR$ and two $ERR^{UL}$ in \textit{All} \textit{Uninformative 1000} or \textit{Ideal 1000} query sets. \Dongji{DONE}}
		\label{table:kendall_conflict_ERR}
		\end{center}
		\vspace{-3mm}
\end{table}




\subsubsection{\bf Statistical Significance Test Yields Different Outcomes for Original \textit{ERR} Vs UL-normalized \textit{ERR}:} We again conducted statistical significance tests for every pair of LETOR methods based on their original $ERR$, $nERR$ and $ERR^{U L}$ scores to see how many times the two metrics disagree on the relative performance between two competing LETOR methods. 



Table~\ref{table:statistical_test_conflict_ERR}  summarizes the number of disagreements between $ERR$, $nERR$ and $ERR^{U L}$ in two data-sets.
We again first look at the results from ``MSLR-WEB30K''. While using all query set, both 
$ERR^{U L}$ find disagreements with original $ERR$ and $nERR$. Additionally, there are more conflicts cases appeared while using \textit{uniformative} query set and less number of conflicts in \textit{Ideal} query set.
However, conflicts results in ``MQ2007'' is more complicated. For instance, based on student's t-test,$ERR^{U L}_{V_2}$ disagreed with original $ERR$ on $11$  pairs of LETOR methods for \textit{Uninformative} query set, while even more  \textbf{14} disagreements for \textit{Ideal} query set. This is very interesting since the impact is more powerful in terms of Ideal query set.
Despite this, given the difference in outcomes and disagreements between the original $ERR$ metric and it's UL-normalized version, we still trying to compare these two metrics in terms of their \textit{Discriminative power} and \textit{Consistency} just like what we did in $nDCG$ and $MAP$.



\begin{table}[!htb]
	\begin{center}
	   
		\begin{tabular}{c||c|c|c|c}\hline
		& \multicolumn{4}{c} {\textbf{Conflict Cases}}\\\cline{2-5}
		{\bf Data-set} & {\bf version }& \textbf{All} & {\bf uniform} & {\bf Ideal} \\\hline\hline
		
		\multirow{4}{*}{\bf MSLR-WEB30K} & ERR and V1 & 16 & 15  & 0    \\\cline{2-5}
		
		& ERR and V2 & 16 & 53 & 1 \\\cline{2-5}
		
		& nERR and V1 & 4 & 9 & 0  \\\cline{2-5}
		& nERR and V2 & 4 & 53 & 1 \\\hline\hline
		
	
		
		\multirow{4}{*} {\bf MQ2007} & ERR and V1 & 1&  0 & 4  \\\cline{2-5}
		
		 & ERR and V2 & 8 &  11 &  14 \\\cline{2-5}
		 & nERR and V1 & 0 & 0 &  1 \\\cline{2-5}
		 & nERR and V2 & 7 & 11 &  13\\\hline\hline
	
		\end{tabular}

		\caption{We used Student's t-test to verify whether statistically significant difference occurred between a pair of LETOR methods while using $ERR$ and $ERR^{U L}$ and counted the total number of disagreements on ``MSLR-WEB30K'' and ``MQ2007'' data-set \Dongji{DONE}}
		\label{table:statistical_test_conflict_ERR}
		\end{center}
		\vspace{-3mm}
\end{table}





\subsubsection{\bf Distinguishability}~\\
Using the aforementioned \textit{Uninformative} and \textit{Ideal} query collections, Table~\ref{table:student_discriminative_ERR} shows some interesting results of these statistical tests for different query sets in `MSLR-WEB10K` and''``MQ2007'' data-sets. Let's first look at ``MSLR-WEB10K''. All four $ERR$ variety can almost detect all ($140$ cases) statistically significant difference. In \textit{uninformative} query set, this \textit{Distinguishability} still hold except $ERR^{U L}_{V_2}$ which can only detect $86$ cases. However, in ``MQ2007'' data-set, $ERR^{U L}_{V_2}$ can detect most number of difference cases ($42$ and $38$) when we using the all query set and  \textit{uninformative} query set respectively. More interesting, even in $Ideal$ query set, $ERR^{U L}_{V_2}$ can still detect $50$ number of cases, which is the most among other three versions.
 
 



\begin{table}[!htb]
	\begin{center}
	   
		\begin{tabular}{c||c|c|c|c}\hline
		& \multicolumn{4}{c} {\textbf{Number of Stat-Sig difference}}\\\cline{2-5}
		{\bf Data-set} & {\bf version }& {\bf All} &{\bf uninform} & {\bf Ideal} \\\hline\hline
		
		\multirow{4}{*}{\bf MSLR-WEB30K} & ERR & 140  & 118 &  140   \\\cline{2-5}
		
		& nERR & 137 & 116 & 135 \\\cline{2-5}
		& V1 &  140 & \textbf{119} & 139\\\cline{2-5}
		& V2 & 140 & \textbf{86} & 140 \\\hline\hline
		
	
		
		\multirow{4}{*} {\bf MQ2007} & ERR & 36 & 35  &  36 \\\cline{2-5}
		
		& nERR & 35 &  35& 41 \\\cline{2-5}
		& V1 &  35 &  35& 40  \\\cline{2-5}
		
		& V2 & 42 & \textbf{38} & 50 \\\hline
	
		\end{tabular}
		
		
		\caption{Total number of statistically significant differences detected based on $ERR$ and $ERR^{UL}$ on all queries, 1000 \textit{uninformative} queries and \textit{Ideal} queries from the ``MSLR-WEB30K'' and `` MQ2007 '' data-set. \Dongji{DONE}}
        \label{table:student_discriminative_ERR}
		\end{center}
		\vspace{-3mm}
\end{table}



Next, we still use the formula ~\ref{equ:pad} to compute the percentage of absolute differences between pairs of LETOR methods in terms of their original $ERR$, $nERR$ and $ERR^{U L}_{V}$, separately. Here, {\bf X} represents $ERR$, $nERR$ and $ERR^{U L}_{V_{1,2}}$. (Details of PAD can be found in ~\ref{sec:nDCG_distin}). 

Table~\ref{tab:ERR_PAD_result} illustrates the PAD score in case of $ERR$ and proposed two $ERR^{U L}$ from two data-sets for different query collections.


From this table, we can still observe that while using $ERR^{U L}$ can achieve higher PAD score than the same for original $MAP$ 
for all types of query collections except for 
$ERR^{U L}_{V_2}$ while using uninformative query from ``MSLR-WEB30K'', in this case, $ERR^{U L}_{V_2}$ achieves the least PAD (27.39). Even $ERR^{U L}_{V_2}$ still achieve a huge improvement in terms of finding the difference for ALL query set in ``MSLR-WEB30K''. This is identical to the observation from Table~\ref{table:student_discriminative_ERR}. Thus, we can attribute this to the limited number of uninformative query set (we only use 1000 among 10,000) and resulting the improvement is still positive using ALL query set.



These results show that the proposed LB normalization 
again improve the distinguishability of original $ERR$ to some extent and can better differentiate between the quality of two LETOR methods  with a larger margin.

\begin{table*}[!htb]
    \begin{adjustbox}{width=0.9\linewidth}
    \centering
    \begin{tabular}{c|c|c||c|c||c|c}\hline 

    & \multicolumn{6}{c}{ \bf PAD score}
    \\\cline{2-7}
    & \multicolumn{2}{c||} {\bf All Query} & \multicolumn {2}{c||} {\bf uninform} & \multicolumn {2}{c} {\bf Ideal} \\\cline{2-7}
    {\textbf{Metrics}} & {\bf MSLR} & {\bf MQ2007} & {\bf MSLR} & {\bf MQ2007} & {\bf MSLR} & {\bf MQ2007}\\ \hline\hline
    
    {\bf  ERR}  & 35.91  & 8.85 & 30.42  & 11.96 & 47.12  &8.31 \\\hline
    
    {\bf  nERR}  & 32.28 &10.18  &  32.7 & 12.32  &  44.87&8.00 \\\hline
    
    
    {$\bf ERR^{UL}_{V_1}$} &  {\bf 39.44 } & {\bf 10.62} &  {\bf 38.49} & {\bf 13.77} &  {\bf 50.67} & {\bf 9.84} \\\hline
     

    {$\bf ERR^{UL}_{V_2}$} &  {\bf118.9 } & {\bf 34.05} &  {\bf 27.39} & {\bf 32.73} &  {\bf75.02 } & {\bf23.14 } \\\hline
     

    %  {\bf  \makecell{Percentage Change \\ between nDCG and $\bf DCG^{U L}$}}  & \textbf{ +84\%} & \textbf{+26\%}\\\hline

    \end{tabular}
    \end{adjustbox}
    \caption{Percentage Absolute Difference between pairs of LETOR methods in terms of average $ERR$ and $ERR^{U L}$ scores. \Dongji{DONE}}
    \label{tab:ERR_PAD_result}
    \vspace{-5mm}
\end{table*}






\subsubsection{\bf Consistency}~\\
This experiment again focuses to compare the relative ranking of LETOR methods in terms of their $ERR$ and $ERR^{UL}$ scores, separately, \textit{across} different data-sets (``MQ2007'' Vs ``MSLR-WEB30K'') as well as \textit{across} \textit{Uninformative} and \textit{Ideal} query collections within the same data-set. We computed \textit{swap rate}~\cite{sakai2006evaluating} to quantify the consistency of rankings induced by $ERR$ and $ERR^{UL}$ metrics across different data-sets.
Table~\ref{table:Swap_Rate_ERR} shows our swap rate results for $ERR$ variant across the two data-sets, ``MSLR-WEB30K'' and ``MQ2007''. 
Same as $MSP^{UL}_{V_2}$ ,$ERR^{UL}_{V_2}$ can also achieve a overall  \textbf{better} swap rate(least score) across a data-sets comparison while considering all query set.



\begin{table}[!htb]
	\begin{center}
	   
		\begin{tabular}{c||c|c|c}\hline
		& \multicolumn{3}{c} {\textbf{Swap Rate}  }\\\cline{2-4}
		{\bf Metric}  & {\bf All} &  {\bf uninform} & {\bf Ideal}\\\hline\hline
		
		{\bf ERR} & 0.39 & 0.2857   &  0.464 \\\hline
		
		{\bf nERR} & 0.35 & 0.357  &  0.464 \\[1ex]\hline
		
		$\bf ERR^{UL}_{V_1}$ &0.39  & 0.357  & 0.464 \\[1ex]\hline
		$\bf ERR^{UL}_{V_2}$ & 0.32 &  0.392 & 0.464\\[1ex]\hline
	
		\end{tabular}
		
		
		\caption{Swap rates between method ranks on \textit{uninform }/\textit{Ideal} queries across ``MSLR-WEB30K'' and ``MQ2007''  data-sets.\Dongji{DONE}}
        \label{table:Swap_Rate_ERR}
		\end{center}
		\vspace{-3mm}
\end{table}
On the other hand, 
Table~\ref{table:Swap_Rate_across_dataset_ERR} also shows our swap rate results for $ERR$ and $ERR^{UL}$ across \textit{Uninformative} Vs \textit{Ideal} queries from the same data-set. Unfortunately, we only see $ERR^{UL}$ make the comparison across query set more inconsistent.

\begin{table}[!htb]
	\begin{center}
	   
		\begin{tabular}{c||c|c}\hline
		& \multicolumn{2}{c} {\textbf{Swap Rate}  }\\\cline{2-3}
		{\bf Metric}  & {\bf MSLR-WEB30K} & {\bf MQ2007}\\\hline\hline
		{\bf ERR} &   0.14& 0.25  \\[1ex]\hline
		{\bf nERR} &   0.25& 0.39  \\[1ex]\hline
		$\bf ERR^{UL}_{V_1}$ &   0.25 & 0.39
		\\[1ex]\hline
		
		$\bf ERR^{UL}_{V_2}$ & 0.39    &  0.32\\[1ex]\hline
	
		\end{tabular}
		\caption{Swap rates between method ranks on \textit{MSLR-WEB30K}/\textit{MQ2007} data-sets across ``uninform'' and ``Ideal'' query collections. \Dongji{DONE}}
        \label{table:Swap_Rate_across_dataset_ERR}
		\end{center}
		\vspace{-3mm}
\end{table}




% \begin{table*}[!htb]
%     \begin{adjustbox}{width=0.9\linewidth}
%     \centering
%     \begin{tabular}{c|c|c||c|c||c|c}\hline 

%     & \multicolumn{6}{c}{ \bf PAD score}
%     \\\cline{2-7}
%     & \multicolumn{2}{c||} {\bf All Query} & \multicolumn {2}{c||} {\bf uninform} & \multicolumn {2}{c} {\bf Ideal} \\\cline{2-7}
%     {\textbf{Metrics}} & {\bf MSLR} & {\bf MQ2007} & {\bf MSLR} & {\bf MQ2007} & {\bf MSLR} & {\bf MQ2007}\\ \hline\hline
    
%     {\bf  ERR}  & 35.91  & 8.85 & 30.42  & 11.96 & 47.12  &8.31 \\\hline
    
%     {\bf  nERR}  & 32.28 &10.18  &  32.7 & 12.32  &  44.87&8.00 \\\hline
    
    
%     {$\bf ERR^{UL}_{V_1}$} &  {\bf 39.44 } & {\bf 10.62} &  {\bf 38.49} & {\bf 13.77} &  {\bf 50.67} & {\bf 9.84} \\\hline
     

%     {$\bf ERR^{UL}_{V_2}$} &  {\bf118.9 } & {\bf 34.05} &  {\bf 27.39} & {\bf 32.73} &  {\bf75.02 } & {\bf23.14 } \\\hline
     

%     %  {\bf  \makecell{Percentage Change \\ between nDCG and $\bf DCG^{U L}$}}  & \textbf{ +84\%} & \textbf{+26\%}\\\hline

%     \end{tabular}
%     \end{adjustbox}
%     \caption{Percentage Absolute Difference between pairs of LETOR methods in terms of average $ERR$ and $ERR^{U L}$ scores. \Dongji{DONE}}
%     \label{tab:ERR_PAD_result}
%     \vspace{-5mm}
% \end{table*}






% \subsubsection{\bf LB Normalization Increases the Percentage Absolute Differences between Two LETOR Methods:} 
% By using the formula~\ref{equation:PAD}, we can compute the difference of average score  with varying cutoff variable $k$ ($k$ is $5,10,15,20,30$) between LETOR methods while using ERR and $ERR^{U L}_{V}$ where in this case, {\bf nDCG} is replaced by $ERR$ and $ERR^{U L}_{V}$.(Details of PAD can be found in ~\ref{sec: nDCG_sd_method difference}).   Table ~\ref{table:UL-ERR_method_percentage_differenceMSLR} shows the details of these percentage differences of various LETOR method pairs in terms of original $ERR$
% while Table~\ref{tab:V1ERR_Letormethod_average_difference_my_label_MSLR} and Table ~\ref{tab:V2ERR_Letormethod_average_difference_my_label_MSLR} show the percentage absolute differences of various LETOR method pairs in terms of $ERR^{U L}_{V}$, on ``MSLR-WEB10K'' data-set. Let us first take a look at the difference between $ERR$  and $ERR^{U L}_{V_1}$. In most cases $ERR^{U L}_{V_1}$ achieves higher PAD scores.However, these differences are not significant, even in some cases that $ERR$ has better performance in terms of distinguishability such as the difference between <RF, LMART>, original $ERR$ has higher value (7.64) compared with $ERR^{U L}_{V_1}$ (4.93). Similar with $ERR^{U L}_{V_1}$, for the particular case <RF, LMART> $ERR^{U L}_{V_2}$ still perform worse than original $ERR$ for distinguishing the difference in between, although for the rest of LETOR method-pairs 
% $ERR^{U L}_{V_2}$ leads to much higher difference. 
% Table~\ref{tab:ERR_PAD_result} concludes these average PAD of all possible LETOR method pairs in terms of original $ERR$ score and $ERR^{U L}_{V}$ score. From this table, we can observe that average $PAD$ of different LETOR method pairs while using $ERR^{U L}_{V}$ is  higher than the same for original $ERR$. At the same time,  $ERR^{U L}_{V_2}$ achieves the highest $PAD$ score in both data-sets(\textbf{91.5 and 34.05}).









% \subsubsection{\bf Statistical Significance Test Yields Different Outcomes for Original \textit{ERR} Vs UL-normalized \textit{ERR}:}
% \texttt{} \label{sec: ERRwilcoxontest}
% For this experiment, we took a closer look at closely performing LETOR method pairs in terms of original \textit{ERR} and conducted statistical significance test (Wilcoxon Signed-Rank Test~\cite{woolson2007wilcoxon}) to verify whether the observed difference has occurred due to mere random fluctuations or not. For example, setting $k=15$, ARank achieves a \textit{ERR} score of $0.2693$ and RBoost achieves a \textit{ERR} score of $0.2433$ (Table~\ref{table:ERRandnERR_averageVaryKMSLR_WEB10K}). Wilcoxon signed-rank test in this case resulted in a p-value of $0.27$, which means the observed difference is not statistically significant assuming a threshold of $0.05$.

% Table~\ref{tab:wilcoxon_scoreERRForMSLR_all} (rows 2 to 6) shows some interesting results of these statistical tests for all queries in ``MSLR-WEB10K'' data-set. Specifically, we consider a particular closely performing LETOR method-pair: <ARank, RBoost>  for this experiment and show the p-value for each particular $k$ of this LETOR method-pair using both traditional $ERR$ and two variants of UL bound normalized $ERR$. Adopting the most widely used confidence value of $0.05$ as the threshold, a p-value larger than $0.05$ means the two distributions are statistically same, otherwise the pair of distributions are statistically different. From this table, we can see that statistical significance test yields different results for original $ERR$ vs. UL bound normalized \textit{ERR}. For instance, for $k=10$,  while Wilcoxon Signed-Rank Test indicates that the methods are not distinguishable in terms of their original $ERR$ scores (p-value = 0.28), the same test indicates the opposite way in case of $ERR^{U L}_{V_2}$ scores (p-value = 0.005). Additionally, for this special pair, $ERR^{U L}_{V_2}$ indicates the opposite results for all $k$ setting (i.e., $k = [5,10,15,20,30]$).  This means that involving a realistic upper lower bound normalization to original \textit{ERR} can lead to different conclusions when comparing two LETOR methods.


% \subsubsection{\bf UL bound Normalization effect on Broad Vs Focused Queries:}\label{sec:utilityERR} \hspace{1mm} Our next experiment again focuses to find special cases where UL bound Normalization may have a more substantial impact. 
% We still leverage the previously defined ``broad'' and ``focused'' query set to check whether we can observe the similar implication in $nDCG$. Table  ~\ref{tab:wilcoxon_scoreERRForMSLR_all} and Table ~\ref{tab:wilcoxon_scoreERRForMQ2007_all} summarized this utility test in our two data-sets. First of all, we can observe that on both data-sets, the number of conflicting cases on ``broad'' query set is higher than ``focused'' query set. For instance, on ``MSLR-WEB10K'' there are \textbf{19} pairs of conflicting method-pairs in broad query set, especially for LMART and RF pair, both $ERR^{U L}_{V_1}$ and $ERR^{U L}_{V_2}$ lead to an opposite conclusion for all $k$ setting. However, only one pairs (L2LR and RNet) exist in focused query set. While on our second data-set ``MQ2007'', though there are totally 3 pairs of conflicting cases in terms of this statistical test, the number of ``broad'' query (\textbf{2} pairs) is still higher than ``focused'' query(\textbf{1} pair), thus, supporting our hypothesis.


% \subsubsection{\bf Impact of LB Normalization on the Metric Variance} \label{sec: averagePerformanceERR}

% Figure ~\ref{fig:ERR_RMSD_MSLR} and ~\ref{fig:ERR_RMSD_MQ2007} depict the Standard Deviation (SD) results for all eight LETOR methods (with respect to varying k) in terms of \textit{ERR}, \textit{nERR} and other two variants of joint upper and lower-bound normalized $ERR$ on two data-sets graphically, where x-axis represents different LETOR methods and the y-axis represents the corresponding SD. These charts more clearly show the lower sensitivity of our both our two upper \& lower-bound normalized $ERR$ compared to the original $ERR$ on our first data-set.While in ``MQ2007'', $ERR^{U L}_{V_2}$ obtains the highest SD .
% However, in all cases, $ERR^{U L}_{V_1}$ obtains the lowest SD on this data-set, such as for LNet, RNet and L2LR from figure ~\ref{fig:ERR_RMSD_MQ2007}. 
% while for $ERR^{U L}_{V_2}$, even we doubled the range (range change from [0,1] to [-1,1]), the SD of $ERR^{U L}_{V_2}$ is still less than original \textit{ERR} on ``MSLR-WEB10K'', such as LNet, RBoost and LMART (in figure ~\ref{fig:ERR_RMSD_MSLR}). However,from figure ~\ref{fig:ERR_RMSD_MQ2007} we can observe that the SD results of $ERR^{U L}_{V_2}$ for all eight LETOR methods are higher than the SD of original $ERR$,  which is also interesting. Overall, our first variant still hold the fact in terms of reducing the sensitivity of LETOR method w.r.t varying $k$.

% \begin{table}
%     \begin{adjustbox}{width=0.5\linewidth}
%     \begin{tabular}{c|c|c|c|c|c}\hline
    
%     \textbf{Query Type} & \textbf{k} & {\bf Methods}  & {\bf ERR} & {\bf V1} & {\bf V2}  \\\hline\hline
    
%     \multirow{5}{*}{\bf MSLR} &  5 &  {ARank \& RBoost}  &  {\bf\textcolor{blue}{0.4}} & 0.18 & {\bf\textcolor{red}{0.001}} \\\cline{2-6}
    
%     &  10 &  {ARank \& RBoost}  &  {\bf\textcolor{blue}{0.28}} & 0.146 & {\bf\textcolor{red}{0.005}} \\\cline{2-6}

%     & 15 & { ARank \& RBoost}  &  {\bf\textcolor{blue}{0.27}} & 0.141  & {\bf\textcolor{red}{0.006}}   \\\cline{2-6}
    
%     & 20 & {ARank \& RBoost}  &  {\bf\textcolor{blue}{0.26}} & 0.143 &  {\bf\textcolor{red}{0.01}}  \\\cline{2-6}
    
%     & 30 & {ARank \& RBoost}  &  {\bf\textcolor{blue}{0.25}} & 0.13 &  {\bf\textcolor{red}{0.01}} \\\hline\hline
    
%     \multirow{6}{*}{\bf MQ2007} &  \multirow{2}{*}{5} &  {CA \& RNet}  &  {\bf\textcolor{red}{0.037}} &{\bf\textcolor{blue}{0.05}} & 0.039 \\\cline{3-6}
    
%     & & {L2LR \& RNet} & {\bf\textcolor{red}{0.042}} &{\bf\textcolor{blue}{0.06 }} & 0.037 \\\cline{2-6}
    
    
%     &15 & { LNet \& RBoost}  &  {\bf\textcolor{red}{0.03}} & {\bf\textcolor{blue}{0.06}}    & {\bf\textcolor{blue}{0.054}}   \\\cline{2-6}
    

    
%     & \multirow{3}{*}{20} & {L2LR \& LNet}  &  {\bf\textcolor{red}{0.043}} &{\bf\textcolor{blue}{0.052}} &  {\bf\textcolor{blue}{0.06}}\\\cline{3-6}
    
%     & & {LNet \& RBoost} & {\bf\textcolor{red}{0.027}} & 0.049 &{\bf\textcolor{blue}{0.053 }}  \\\cline{3-6}
    
%      & & {RBoost \& RNet} & {\bf\textcolor{red}{0.038}} & {\bf\textcolor{blue}{0.05 }} & {\bf\textcolor{blue}{0.066 }}  \\\hline\hline
    
    
    
%     \end{tabular}
%     \end{adjustbox}
%     \caption{p-Values for Wilcoxon Signed-Rank Test performed on pairs of LETOR methods. We used $0.05$ as our threshold; red and blue color highlights cases where the same test gives different outcomes. MQ2007  \textbf{DONE}}
%     \label{tab:wilcoxon_score_ERR_For_MSLR_MQ2007_all}
% \end{table}




% \begin{table}
%     \begin{adjustbox}{width=0.5\linewidth}
%     \begin{tabular}{c|c|c|c|c|c}\hline
    
%     \textbf{Query Type} & \textbf{k} & {\bf Methods}  & {\bf ERR} & {\bf V1} & {\bf V2}  \\\hline\hline
    
    
%     % \multirow{5}{*}{\bf All} &  5 &  {ARank \& RBoost}  &  {\bf\textcolor{blue}{0.4}} & 0.18 & {\bf\textcolor{red}{0.001}} \\\cline{3-6}
    
%     % &  10 &  {ARank \& RBoost}  &  {\bf\textcolor{blue}{0.28}} & 0.146 & {\bf\textcolor{red}{0.005}} \\\cline{3-6}

%     % & 15 & { ARank \& RBoost}  &  {\bf\textcolor{blue}{0.27}} & 0.141  & {\bf\textcolor{red}{0.006}}   \\\cline{3-6}
    
%     % & 20 & {ARank \& RBoost}  &  {\bf\textcolor{blue}{0.26}} & 0.143 &  {\bf\textcolor{red}{0.01}}  \\\cline{3-6}
    
%     % & 30 & {ARank \& RBoost}  &  {\bf\textcolor{blue}{0.25}} & 0.13 &  {\bf\textcolor{red}{0.01}} \\\hline\hline
    

%     \multirow{14}{*}{\bf Broad} & \multirow{3}{*}{5} & {LMART \& RF} & {\bf\textcolor{red}{0.031}} & {\bf\textcolor{blue}{0.051 }}  & {\bf\textcolor{blue}{0.11 }} \\\cline{3-6}
    
%     & & {ARank \& RBoost} & {\bf\textcolor{red}{0.004}} & 0.025 &{\bf\textcolor{blue}{0.3 }}  \\\cline{3-6}
    
%     & & {LNet \& RNet} & {\bf\textcolor{red}{0.026}} &  0.02 &{\bf\textcolor{blue}{0.05 }}  \\\cline{2-6}

    
%     & \multirow{2}{*}{10} & {LMART \& RF}  & {\bf\textcolor{red}{0.035}}   &{\bf\textcolor{blue}{0.06}} & {\bf\textcolor{blue}{0.11}}  \\\cline{3-6}

        
%     & & {ARank \& RBoost} & {\bf\textcolor{red}{0.01}} & 0.04  &{\bf\textcolor{blue}{0.23 }}  \\\cline{2-6}
    
%     &\multirow{3}{*}{15} &  {LMART \& RF}  & {\bf\textcolor{red}{0.04}} & {\bf\textcolor{blue}{0.07}} &  {\bf\textcolor{blue}{0.11}}\\\cline{3-6}
    
%     & & {ARank \& RBoost} & {\bf\textcolor{red}{0.013}} & 0.043  &{\bf\textcolor{blue}{0.23 }}  \\\cline{3-6}
    
%     & & {LNet \& RNet} & {\bf\textcolor{red}{0.04}} &  0.03 &{\bf\textcolor{blue}{0.056 }}  \\\cline{2-6}
    

%     & \multirow{3}{*}{20} & {LMART \& RF} &{\bf\textcolor{red}{0.04}}& {\bf\textcolor{blue}{0.06}} & {\bf\textcolor{blue}{0.1}}  \\\cline{3-6}
    
    
%     & & {ARank \& RBoost} & {\bf\textcolor{red}{0.01}} &  0.043 &{\bf\textcolor{blue}{0.23 }}  \\\cline{3-6}
%     & & {LNet \& RNet} & {\bf\textcolor{red}{0.49}} & 0.037  &{\bf\textcolor{blue}{0.1 }}  \\\cline{2-6}
    
%     & \multirow{3}{*}{30} & {LMART \& RF} &{\bf\textcolor{red}{0.03}}& {\bf\textcolor{blue}{0.058}} & {\bf\textcolor{blue}{0.09}}  \\\cline{3-6}

%     & & {ARank \& RBoost} & {\bf\textcolor{red}{0.01}} & 0.044  &{\bf\textcolor{blue}{0.22 }}  \\\cline{3-6}
%     & & {LNet \& RNet} & {\bf\textcolor{red}{0.04}} & 0.032  &{\bf\textcolor{blue}{0.05 }}  \\\hline\hline

%     \multirow{1}{*}{\bf Focused} & 5 & {L2LR \& RNet} & {\bf\textcolor{red}{0.018}} & 0.04 &{\bf\textcolor{blue}{0.23}} \\\hline

%     % & 30 & {LMART \& RNet} & {\bf\textcolor{red}{0.04}} &{\bf\textcolor{blue}{0.08}} & 0.03 \\\hline   
    
    
    
%     \end{tabular}
%     \end{adjustbox}
%     \caption{p-Values for Wilcoxon Signed-Rank Test performed on pairs of LETOR methods. We used $0.05$ as our threshold; red and blue color highlights cases where the same test gives different outcomes. MSLR-WEB10K DONE}
%      \label{tab:wilcoxon_scoreERRForMSLR_all}
% \end{table}




% \begin{table}
%     \begin{adjustbox}{width=0.5\linewidth}
%     \begin{tabular}{c|c|c|c|c|c}\hline
    
%     \textbf{Query Type} & \textbf{k} & {\bf Methods}  & {\bf ERR} & {\bf V1} & {\bf V2}  \\\hline\hline
    
    
%     % \multirow{6}{*}{\bf All} &  \multirow{2}{*}{5} &  {CA \& RNet}  &  {\bf\textcolor{red}{0.037}} &{\bf\textcolor{blue}{0.05}} & \\\cline{3-6}
    
%     % & & {L2LR \& RNet} & {\bf\textcolor{red}{0.042}} &{\bf\textcolor{blue}{0.06 }} & \\\cline{2-6}
    
    
%     % &15 & { LNet \& RBoost}  &  {\bf\textcolor{red}{0.03}} & {\bf\textcolor{blue}{0.06}}    & {\bf\textcolor{blue}{0.06}}   \\\cline{2-6}
    

    
%     % & \multirow{3}{*}{20} & {L2LR \& LNet}  &  {\bf\textcolor{red}{0.043}} &{\bf\textcolor{blue}{0.052}} &  {\bf\textcolor{blue}{0.06}}\\\cline{3-6}
    
%     % & & {LNet \& RBoost} & {\bf\textcolor{red}{0.027}} & &{\bf\textcolor{blue}{0.053 }}  \\\cline{3-6}
    
%     %  & & {RBoost \& RNet} & {\bf\textcolor{red}{0.038}} & & {\bf\textcolor{blue}{0.066 }}  \\\hline\hline
    
%     \multirow{2}{*}{\bf Broad} & 5 & {RBoost \& RNet} & {\bf\textcolor{blue}{0.077}}    &{\bf\textcolor{red}{0.045 }} &  0.055\\\cline{2-6}
    
%     & 10 & {LMART \& RNet} & {\bf\textcolor{blue}{0.16}}  & 0.09 &{\bf\textcolor{red}{0.044 }}\\\hline\hline
  
%     {\bf Focused} & 10 & {CA \& RBoost} & {\bf\textcolor{blue}{0.06}} & 0.063 &{\bf\textcolor{red}{0.03}} \\\hline 

    
    
%     \end{tabular}
%     \end{adjustbox}
%     \caption{p-Values for Wilcoxon Signed-Rank Test performed on pairs of LETOR methods. We used $0.05$ as our threshold; red and blue color highlights cases where the same test gives different outcomes. MQ2007  \textbf{DONE}}
%     \label{tab:wilcoxon_scoreERRForMQ2007_all}
% \end{table}


% \begin{figure}[!htb]
%     \vspace{-3mm}
%     \centering
%     \includegraphics[width=0.5\linewidth]{figs/ERR/figs/ERR_MSLR.png}
%     \vspace{-4mm}
%     \caption{Standard Deviation of Different ERR Variants for eight LETOR methods on MSLR-WEB10K data-set}
%     \label{fig:ERR_RMSD_MSLR}
%     % \vspace{-4mm}
% \end{figure}


% \begin{figure}[!htb]
%     % \vspace{-3mm}
%     \centering
%     \includegraphics[width=0.5\linewidth]{figs/ERR/figs/ERR_MQ2007.png}
%     \vspace{-3mm}
%     \caption{Standard Deviation of Different ERR Variants for eight LETOR methods on MQ2007 data-set}
%     \label{fig:ERR_RMSD_MQ2007}
%     \vspace{-4mm}
% \end{figure}

% Table ~\ref{tab:ERRwilcoxon_score} shows for this pair of methods no matte what value we take for ，they are always statistically same with each other as their p-value is always higher than our assuming a threshold of $0.05$. However, after using $ERR^{U L}_{V_3}$, the p-value is always less than $0.05$ which means the distributions are statistically different.


% Table ~\ref{tab:ERRwilcoxon_score} summarized the wilcixon signed-tank test result for $ERR$. Compared with $nDCG$, involving upper \& lower bound normalization for ERR leads to a more uniform result: for ListNet and RankNet pair, $ERR^{U L}_{V_3}$ always amplifies the statistically significant difference between each other.



% \begin{table}\footnotesize
%     \begin{adjustbox}{width=0.6\linewidth}

%     \begin{tabular}{c|c|c|c|c}\hline
    
%     {\bf Methods}  & {\bf ERR} & {\bf V1} & {\bf V2} & {\bf V3} \\\hline\hline
%     & \multicolumn{4}{c}{\bf K = 5} \\\cline{1-5}
%     {LNet \& RNet}  & {\bf\textcolor{blue}{0.0502}} & 0.058  & 0.072 & {\bf \textcolor{red}{0.006}}\\\hline
    
    
%     & \multicolumn{4}{c}{\bf K = 10} \\\cline{1-5}
    
%     {LNet \& RNet} & {\bf\textcolor{blue}{0.0667}} & 0.085  & 0.085 & {\bf\textcolor{red}{0.0097}} \\\hline
    
    
%     & \multicolumn{4}{c}{\bf K = 15} \\\cline{1-5}
%     {LNet \& RNet} & {\bf\textcolor{blue}{0.1035}} & 0.1265  & 0.128 & {\bf\textcolor{red}{0.0067}} \\\hline
    
    
%     & \multicolumn{4}{c}{\bf K = 20} \\\cline{1-5}
%     {LNet \& RNet} & {\bf\textcolor{blue}{0.144}} &0.171 &0.175 & {\bf \textcolor{red}{0.007}}\\\hline
    
    
%     & \multicolumn{4}{c}{\bf K = 30} \\\cline{1-5}
    
%     {LNet \& RNet} &{\bf\textcolor{blue}{0.1502}} & 0.1793 & 0.179 & {\bf \textcolor{red}{0.0073}}  \\\hline
    
    
%     \end{tabular}
%     \end{adjustbox}
%     \caption{p-Values for Wilcoxon Signed-Rank Test performed on pairs of LETOR methods with comparable performance. We used $0.05$ as our threshold; red and blue color highlights cases where the same test gives different outcomes.}
%     \label{tab:ERRwilcoxon_score}
% \end{table}

==> sections/Abstract.tex <==
\begin{abstract}
Empirical evaluation is a key challenge for any Information Retrieval (IR) system. Traditionally, some commonly used evaluation metrics for evaluating the quality/ performance of an IR system include \textbf{N}ormalized \textbf{D}iscounted \textbf{C}umulative \textbf{G}ain ($nDCG$),  \textbf{E}xpected \textbf{R}eciprocal \textbf{R}ank ($ERR$), \textbf{M}ean \textbf{A}verage \textbf{P}recision ($MAP$) etc. Due to the nature of IR applications, the success of a retrieval system depends on the user's satisfaction; thus, an accurate and fair evaluation metric is very important for measuring the perceived utility of a retrieval system by the real users. Unfortunately, ensuring fairness is non-trivial and evaluation metrics often suffer from implicit biases and inaccurate assumptions. For example, conventional $nDCG$ and $MAP$ metrics only include query-specific upper-bound normalization, but no query-specific lower-bound normalization. On the other hand, for $ERR$, there is no query-specific upper or lower bound normalization. But each query is diverse in terms of its complexity, user intent, distribution of relevance labels of its related documents, and user's perceived utility at different cut-off rank $k$, implying that the measure should account for both query-specific upper and lower-bounds. Otherwise, the metric will fail to correctly capture the \textit{real} learning quality of a ranker and thus, will result in unfair comparison across multiple queries and numerous ranking systems.



In this paper, we propose a new general framework with both Upper and Lower bound \textbf{(ULB)} normalization to ensure fairer IR evaluation and then, instantiate the new framework for three popular IR evaluation metrics: $nDCG$, $ERR$, $MAP$. We further introduce three distinct variations of the proposed query-specific joint upper \& lower bound normalization for each metric, yielding a total of nine new metrics, and also compare them to the corresponding traditional metrics without the proposed normalization. Another significant contribution of this paper is that we demonstrate how to compute more realistic query-specific lower-bounds for different evaluation metrics by computing their expected values for each query in the case of a randomized ranking of the related documents; and also theoretically prove their correctness. 





Experiments with eight Learning-to-rank (LETOR) methods revealed that our new ULB evaluation framework (joint upper \& lower bound normalization) demonstrated the following properties: 1) ULB normalization has a significant impact on the original corresponding metrics resulting in \textbf{21-35}\% drop in terms of its average value for eight LETOR methods. 2) ULB metrics are less sensitive \textbf{(more robust)} to the variation of cut-off $k$ resulting in a \textbf{68\%} decrease in average Standard Deviation (SD) w.r.t. varying $k$ across all LETOR methods, 3) While reduction of SD is observed across all the queries for any LETOR method \textbf{(more general)}, percentage differences among multiple LETOR methods actually increase \textbf{(more distinguishable)}, 4) For a number of closely performing LETOR method-pairs, \textbf{statistically significant} differences in terms of original metrics (nDCG, ERR, MAP)  \textbf{no longer} remain statistically significant in terms of ULB normalized \textit{nDCG}, \textit{ERR}, \textit{MAP} and vice-versa. Therefore, we suggest the community to rethink about the current practice of evaluating IR systems and transition to ULB normalized evaluation from now on.
\end{abstract}
